Scaling Laws for Galaxy Images

We present the first systematic investigation of supervised scaling laws outside of an ImageNet-like context - on images of galaxies. We use 840k galaxy images and over 100M annotations by Galaxy Zoo volunteers, comparable in scale to Imagenet-1K. We find that adding annotated galaxy images provides a power law improvement in performance across all architectures and all tasks, while adding trainable parameters is effective only for some (typically more subjectively challenging) tasks. We then compare the downstream performance of finetuned models pretrained on either ImageNet-12k alone vs. additionally pretrained on our galaxy images. We achieve an average relative error rate reduction of 31% across 5 downstream tasks of scientific interest. Our finetuned models are more label-efficient and, unlike their ImageNet-12k-pretrained equivalents, often achieve linear transfer performance equal to that of end-to-end finetuning. We find relatively modest additional downstream benefits from scaling model size, implying that scaling alone is not sufficient to address our domain gap, and suggest that practitioners with qualitatively different images might benefit more from in-domain adaption followed by targeted downstream labelling.

==> spare.tex <==


% \paragraph{Preprint option}
% If you wish to post a preprint of your work online, e.g.\, on arXiv, using the
% NeurIPS style, please use the \verb+preprint+ option. This will create a
% nonanonymized version of your work with the text ``Preprint. Work in progress.''
% in the footer. This version may be distributed as you see fit, as long as you do not say which conference it was submitted to. Please \textbf{do
%   not} use the \verb+final+ option, which should \textbf{only} be used for
% papers accepted to NeurIPS. 



% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to break the
% lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% authors names on the first line, and the last on the second line, try using
% \AND instead of \And before the third author name.

% \thanks{Use footnote for providing further information
%     about author (webpage, alternative address)---\emph{not} for acknowledging
%     funding agencies.} 


% \author{Mike Walmsley$^{1}$, Micah Bowles, Anna M.M.\ Scaife, Jason Shingirai Makechemu,\\\bf Alexander J. Gordon, Annette M.~N.~Ferguson, Robert G.~ Mann, James Pearson,\\\bf Jürgen J. Popp, Jo Bovy, Josh Speagle, Hugh Dickinson, Lucy Fortson,\\\bf Tobias G\'eron,Sandor Kruk, Chris J.\ Lintott, Kameswara Mantha\\\bf Devina Mohan, David O'Ryan, Inigo V.\ Slijepevic}



% % TODO email may be optional?
% \author{%
%   Mike Walmsley\\
%   Dunlap Institute\\
%   University of Toronto\\
%   Toronto, ON M5S 3H4\\
%   \texttt{m.walmsley@utoronto.ca} \\
%   \And
%   Micah Bowles \\
%   Affiliation \\
%   Address \\
%   \texttt{email} \\
%   \AND
%   Anna M.M.\ Scaife \\
%   Affiliation \\
%   Address \\
%   \texttt{email} \\
%   \And
%   Jason Shingirai Makechemu \\
%   Department of Physics \\
%   Lancaster University \\
%   Bailrigg, Lancaster LA1 4YW \\
%   \texttt{j.makechemu@lancaster.ac.uk} \\
%       \And
%     Alexander J. Gordon\\
%         Institute for Astronomy, University of Edinburgh \\
%     Royal Observatory, Blackford Hill, Edinburgh, EH9 3HJ, UK \\
%     \texttt{alexander.gordon@ed.ac.uk} \\
%     \And
%         Annette M.~N.~Ferguson\\
%     Institute for Astronomy, University of Edinburgh\\
%     Blackford Hill, Edinburgh UK EH9 3HJ \\
%     \texttt{annette.ferguson@ed.ac.uk} \\
%     \And
%     Robert G. Mann\\
%   Institute for Astronomy, University of Edinburgh\\
%     Royal Observatory, Blackford Hill,\\ Edinburgh, EH9 3HJ, UK\\ 
%     \texttt{rgm@roe.ac.uk} \\
%   \And
%   James Pearson \\
%   Affiliation \\
%   Address \\
%   \texttt{email} \\
%     \And
%   Jürgen J. Popp \\
%   School of Physical Sciences, The Open University \\
%   Walton Hall, Milton Keynes, MK7 6AA \\
%   \texttt{jurgen.popp@open.ac.uk} \\
%     \And
%   Jo Bovy \\
%   Department of Astronomy \& Astrophysics\\
%   University of Toronto\\
%   Toronto, ON M5S 3H4\\
%   \texttt{jo.bovy@utoronto.ca} \\
%     \And
%   Josh Speagle \\
%   Affiliation \\
%   Address \\
%   \texttt{email} \\
%     \And
%   Hugh Dickinson \\
%   School of Physical Sciences, The Open University \\
%   Walton Hall, Milton Keynes, MK7 6AA \\
%   \texttt{hugh.dickinson@open.ac.uk} \\
%     \And
%   Lucy Fortson \\
%   School of Physics and Astronomy \\
%   Minnesota Institute for Astrophysics \\
%   University of Minnesota \\
%   Minneapolis, MN 55455 \\
%   \texttt{lfortson@umn.edu} \\
%     \And
%   Tobias G\'eron \\
%   Dunlap Institute for Astronomy \& Astrophysics \\
%   University of Toronto \\
%   Toronto, ON M5S 3H4 \\
%   \texttt{tobias.geron@utoronto.ca} \\
%    \And
%   Sandor Kruk \\
%   European Space Agency\\
%   European Space Astronomy Centre (ESAC)\\
%   Camino Bajo del Castillo s/n, 28692\\
%   Villanueva de la Can\~ada, Madrid, Spain\\
%   \texttt{sandor.kruk@esa.int} \\
%    \And
%     Chris J.\ Lintott \\
%   Affiliation \\
%   Address \\
%   \texttt{email} \\
%   \And
%       Kameswara Mantha \\
%   School of Physics and Astronomy \\
%   Minnesota Institute for Astrophysics \\
%   University of Minnesota \\
%   Minneapolis, MN 55455 \\
%   \texttt{manth145@umn.edu} \\
%    \And
%     Devina Mohan \\
%   Department of Physics \& Astronomy\\
%   University of Manchester \\
%   Manchester, M13 9PL, UK \\
%   \texttt{devina.mohan@postgrad.manchester.ac.uk} \\
%    \And
%     David O'Ryan \\
%   Affiliation \\
%   Address \\
%   \texttt{email} \\
%    \And
%     Inigo V.\ Slijepevic \\
%   Affiliation \\
%   Address \\
%   \texttt{email} \\
% }


% In principle, larger models should do no worse (as they could learn the same relation as smaller models); in practice, we see a drop in performance for the very largest models. Fig \ref{fig:overfitting_curves} suggests this may be due to within-epoch overfitting, which larger models are more likely to suffer from given our fixed learning rate (Sec. \ref{sec:limitations}). 



% % Unlike supervised scaling laws, which are broadly untested beyond ImageNet-like images, 
% Transfer learning from ImageNet or other generic data to qualitatively different images
% % has been heavily investigated for medical imaging, where pretraining 
% is `routine' , `pervasive' \cite{}, `integral...the present standard' in the field of medical imaging. The benefit of transfer learning across this domain gap is controversial and likely dataset-dependent \cite{matsoukas_what_2022}.
% % , with e.g.\ no improvement on large downstream datasets [Raghu] but reported benefits when downstream datasets are smaller and more similar [Matsoukas]. 
% Nonetheless, pretraining on large ImageNet-like datasets has been observed to sometimes outperform pretraining on the largest (but far smaller) medical datasets \cite{mustafa_supervised_2021, cherti_effect_2021}. 
% \citet{albarqouni_systematic_2021} experiment with an intermediate in-domain pretraining step, applying additional training on a large in-domain dataset \cite{irvin_chexpert_2019, wang_chestx-ray8_2017} before finetuning to the downstream task, and find (minor) benefits over ImageNet alone. 




% We share a brief investigation below.

% \begin{figure}
%     \centering
%     \includegraphics{figures/finetuned/finetuning_decals10.pdf}
%     \caption{Finetuned performance on the Galaxy10 DECaLS toy dataset}
%     \label{fig:finetuned_decals10}
% \end{figure}


%  We discuss the possible limitations of Galaxy10 in Sec. \ref{sec:galaxy10_limitations}.

% \section{Galaxy10 DECaLS Dataset Limitations}
% \label{sec:galaxy10_limitations}

% Our performance on Galaxy10 DECaLS is excellent for practical use (90\% top-1 accuracy) and compares well to the literature generally, but two very recent works claim 94 and 95\% accuracy \cite{dagli_astroformer_2023,pandya_e2_2023} (one via model scaling with regularisation, and one via equivariance). This paper aims to improve general downstream peformance across a range of tasks, and not on careful tuning for any specific task. However, we believe the Galaxy10 DECaLS dataset may have some specific limitations that make further accuracy improvements difficult.

% Figure \ref{fig:decals10_confusion} shows a typical confusion matrix. 
% Two-thirds of the prediction `errors' (6\% of the dataset) are made on three questions; tight spiral, loose spiral and merger. There is substantial confusion between tight and loose spirals and between loose spiral and mergers. 

% With respect to tight vs. loose spirals, there is an intrinsic overlap between what volunteers describe as tight or loose. Fig \ref{fig:spirals} shows random images where the model predicted `tight' where the label was `loose'. With respect to loose spirals and mergers, the tidal tails formed in mergers often resemble loose spiral arms, and this causes a similar overlap.

% Two further issues affect the dataset in general; duplicates and limited label precision.

% Duplicates are galaxies which appear multiple times. Duplicates cause train/test contamination and may exaggerate the performance of high-capacity models through memorisation. We have traced the source of the duplicates to the telescope software used to identify individual galaxies in large patches of sky. Each image is centered on pixels that the software identified as a galaxy. The software may incorrectly identifying several components of one galaxy as separate galaxies. Images are then created of these `galaxies' (actually one galaxy, repeated with slightly different centering) and labelled and included in Galaxy10 DECaLS. Additionally, when two galaxies are next to one another on the sky (i.e. when they are merging), they also appear in one anothers' images. 
% We can identify likely duplicates by searching for images where the sky coordinates overlap; we estimate approx. 1\% of images are duplicates.

% Limited label precision (as noted by the dataset creators) is an issue because some classes are intrinsically far more common than others. Despite the filtering to confident labels, occasional errors where a highly common class is labelled as a rare class `slip through'. Figure \ref{fig:smooth_disturbed} highlights this issue with galaxies `incorrectly' predicted as smooth when labelled as merger, despite mostly being smooth (as judged by the authors).

% \begin{figure}
%     \centering
%     \includegraphics[width=0.6\textwidth]{figures/cm.png}
%     \caption{Typical DECaLS confusion matrix}
%     \label{fig:decals10_confusion}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{figures/spirals.png}
%     \caption{Spirals with `incorrect' predictions}
%     \label{fig:spirals}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{figures/smooth_disturbed.png}
%     \caption{Galaxies `incorrectly' predicted as disturbed}
%     \label{fig:spirals}
% \end{figure}
